Photon-Limited Blind Deconvolution using Unsupervised Iterative Kernel Estimation

Blind deconvolution is a challenging problem, but in low-light it is even more difficult. Existing algorithms, both classical and deep-learning based, are not designed for this condition. When the photon shot noise is strong, conventional deconvolution methods fail because (1) the image does not have enough signal-to-noise ratio to perform the blur estimation; (2) While deep neural networks are powerful, many of them do not consider the forward process. When the noise is strong, these networks fail to simultaneously deblur and denoise; (3) While iterative schemes are known to be robust in the classical frameworks, they are seldom considered in deep neural networks because it requires a differentiable non-blind solver. This paper addresses the above challenges by presenting an \emph{unsupervised} blind deconvolution method. At the core of this method is a reformulation of the general blind deconvolution framework from the conventional image-kernel alternating minimization to a purely kernel-based minimization. This kernel-based minimization leads to a new iterative scheme that backpropagates an unsupervised loss through a pre-trained non-blind solver to update the blur kernel. Experimental results show that the proposed framework achieves superior results than state-of-the-art blind deconvolution algorithms in low-light conditions.

==> commands2.tex <==
% Common commands and definitions


% *** GRAPHICS RELATED PACKAGES ***
%
%\ifCLASSINFOpdf
%  \usepackage[pdftex]{graphicx}
%  % declare the path(s) where your graphic files are
%  % \graphicspath{{../pdf/}{../jpeg/}}
%  % and their extensions so you won't have to specify these with
%  % every instance of \includegraphics
%  % \DeclareGraphicsExtensions{.pdf,.jpeg,.png}
%\else
%  % or other class option (dvipsone, dvipdf, if not using dvips). graphicx
%  % will default to the driver specified in the system graphics.cfg if no
%  % driver is specified.
%  % \usepackage[dvips]{graphicx}
%  % declare the path(s) where your graphic files are
%  % \graphicspath{{../eps/}}
%  % and their extensions so you won't have to specify these with
%  % every instance of \includegraphics
%  % \DeclareGraphicsExtensions{.eps}
%\fi

\usepackage[colorlinks]{hyperref}
\usepackage{multirow}
\usepackage{times}
\usepackage{amsmath,amssymb}
\usepackage{algorithm}
\usepackage{epstopdf}
\usepackage{subfigure}
\usepackage[dvipsnames]{xcolor}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{cite}
\usepackage{fancyvrb}


%\usepackage{psfrag}
\usepackage{bbm}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{remark}{Remark}
\newtheorem{property}{Property}
\newtheorem{conjecture}{Conjecture}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{condition}{Condition}
\newtheorem{fact}{Fact}
\newtheorem{procedure}{Procedure}
\newtheorem{assumption}{Assumption}
\newenvironment{proof}{\paragraph*{Proof}}{\hfill$\square$}




\newenvironment{densitemize}%    Densely printed itemized list,
{\begin{list}               %    with flush left bullets.
    {$\bullet$ \hfill}{
        \setlength{\leftmargin}{\parindent}
        \setlength{\parsep}{0.04\baselineskip}
        \setlength{\itemsep}{0.5\parsep}
        \setlength{\labelwidth}{\leftmargin}
        \setlength{\labelsep}{0em}}
    }
{\end{list}}

\providecommand{\eref}[1]{\eqref{#1}}  % call \eqref from amstex
\providecommand{\cref}[1]{Chapter~\ref{#1}}
\providecommand{\sref}[1]{Section~\ref{#1}}
\providecommand{\fref}[1]{Figure~\ref{#1}}
\providecommand{\tref}[1]{Table~\ref{#1}}
\providecommand{\thref}[1]{Theorem~\ref{#1}}

\providecommand{\R}{\ensuremath{\mathbb{R}}}
\providecommand{\I}{\ensuremath{\mathbb{I}}}
\providecommand{\C}{\ensuremath{\mathbb{C}}}
\providecommand{\E}{\ensuremath{\mathbb{E}}}
\providecommand{\N}{\ensuremath{\mathbb{N}}}
\providecommand{\Z}{\ensuremath{\mathbb{Z}}}
\providecommand{\Pb}{\ensuremath{\mathbb{P}}}

\providecommand{\bfP}{\mathbf{P}}

\providecommand{\abs}[1]{\lvert#1\rvert}
\providecommand{\norm}[1]{\lVert#1\rVert}
\providecommand{\inprod}[1]{\langle#1\rangle}
\providecommand{\set}[1]{$\left\{#1\right\}$}
\providecommand{\seq}[1]{$\left<#1\right>$}
\providecommand{\bydef}{\overset{\text{def}}{=}}

\renewcommand{\vec}[1]{\ensuremath{\boldsymbol{#1}}}
\providecommand{\mat}[1]{\ensuremath{\boldsymbol{#1}}}




% Some calligraphic letters
\providecommand{\calA}{\mathcal{A}}
\providecommand{\calB}{\mathcal{B}}
\providecommand{\calC}{\mathcal{C}}
\providecommand{\calD}{\mathcal{D}}
\providecommand{\calE}{\mathcal{E}}
\providecommand{\calF}{\mathcal{F}}
\providecommand{\calG}{\mathcal{G}}
\providecommand{\calH}{\mathcal{H}}
\providecommand{\calI}{\mathcal{I}}
\providecommand{\calJ}{\mathcal{J}}
\providecommand{\calK}{\mathcal{K}}
\providecommand{\calL}{\mathcal{L}}
\providecommand{\calM}{\mathcal{M}}
\providecommand{\calN}{\mathcal{N}}
\providecommand{\calO}{\mathcal{O}}
\providecommand{\calP}{\mathcal{P}}
\providecommand{\calQ}{\mathcal{Q}}
\providecommand{\calR}{\mathcal{R}}
\providecommand{\calS}{\mathcal{S}}
\providecommand{\calT}{\mathcal{T}}
\providecommand{\calU}{\mathcal{U}}
\providecommand{\calV}{\mathcal{V}}
\providecommand{\calW}{\mathcal{W}}
\providecommand{\calX}{\mathcal{X}}
\providecommand{\calY}{\mathcal{Y}}
\providecommand{\calZ}{\mathcal{Z}}


% Common matrices and vectors
\providecommand{\mA}{\mathbf{A}}
\providecommand{\mB}{\mathbf{B}}
\providecommand{\mC}{\mathbf{C}}
\providecommand{\mD}{\mathbf{D}}
\providecommand{\mE}{\mathbf{E}}
\providecommand{\mF}{\mathbf{F}}
\providecommand{\mG}{\mathbf{G}}
\providecommand{\mH}{\mathbf{H}}
\providecommand{\mI}{\mathbf{I}}
\providecommand{\mJ}{\mathbf{J}}
\providecommand{\mK}{\mathbf{K}}
\providecommand{\mL}{\mathbf{L}}
\providecommand{\mM}{\mathbf{M}}
\providecommand{\mN}{\mathbf{N}}
\providecommand{\mO}{\mathbf{O}}
\providecommand{\mP}{\mathbf{P}}
\providecommand{\mQ}{\mathbf{Q}}
\providecommand{\mR}{\mathbf{R}}
\providecommand{\mS}{\mathbf{S}}
\providecommand{\mT}{\mathbf{T}}
\providecommand{\mU}{\mathbf{U}}
\providecommand{\mV}{\mathbf{V}}
\providecommand{\mW}{\mathbf{W}}
\providecommand{\mX}{\mathbf{X}}
\providecommand{\mY}{\mathbf{Y}}
\providecommand{\mZ}{\mathbf{Z}}

\providecommand{\va}{\mathbf{a}}
\providecommand{\vb}{\mathbf{b}}
\providecommand{\vc}{\mathbf{c}}
\providecommand{\vd}{\mathbf{d}}
\providecommand{\ve}{\mathbf{e}}
\providecommand{\vf}{\mathbf{f}}
\providecommand{\vg}{\mathbf{g}}
\providecommand{\vh}{\mathbf{h}}
\providecommand{\vi}{\mathbf{i}}
\providecommand{\vj}{\mathbf{j}}
\providecommand{\vk}{\mathbf{k}}
\providecommand{\vl}{\mathbf{l}}
\providecommand{\vm}{\mathbf{m}}
\providecommand{\vn}{\mathbf{n}}
\providecommand{\vo}{\mathbf{o}}
\providecommand{\vp}{\mathbf{p}}
\providecommand{\vq}{\mathbf{q}}
\providecommand{\vr}{\mathbf{r}}
\providecommand{\vs}{\mathbf{s}}
\providecommand{\vt}{\mathbf{t}}
\providecommand{\vu}{\mathbf{u}}
\providecommand{\vv}{\mathbf{v}}
\providecommand{\vw}{\mathbf{w}}
\providecommand{\vx}{\mathbf{x}}
\providecommand{\vy}{\mathbf{y}}
\providecommand{\vz}{\mathbf{z}}



% Greek Matrix bold
\providecommand{\mDelta}{\mat{\Delta}}
\providecommand{\mGamma}{\mat{\Gamma}}
\providecommand{\mLambda}{\mat{\Lambda}}
\providecommand{\mOmega}{\mat{\Omega}}
\providecommand{\mPhi}{\mat{\Phi}}
\providecommand{\mPi}{\mat{\Pi}}
\providecommand{\mPsi}{\mat{\Psi}}
\providecommand{\mSigma}{\mat{\Sigma}}
\providecommand{\mTheta}{\mat{\Theta}}
\providecommand{\mXi}{\mat{\Xi}}
\providecommand{\mSigmaNLM}{\mat{\Sigma}_{\mathrm{NLM}}}
\providecommand{\mSigmahat}{\mat{\widehat{\Sigma}}}

% Greeks Vector bold
\providecommand{\w}{\omega}
\providecommand{\valpha}{\vec{\alpha}}
\providecommand{\vbeta}{\vec{\beta}}
\providecommand{\vgamma}{\vec{\gamma}}
\providecommand{\vdelta}{\vec{\delta}}
\providecommand{\vepsilon}{\vec{\epsilon}}
\providecommand{\vvarepsilon}{\vec{\varepsilon}}
\providecommand{\vzeta}{\vec{\zeta}}
\providecommand{\veta}{\vec{\eta}}
\providecommand{\vtheta}{\vec{\theta}}
\providecommand{\vkappa}{\vec{\kappa}}
\providecommand{\vlambda}{\vec{\lambda}}
\providecommand{\vmu}{\vec{\mu}}
\providecommand{\vnu}{\vec{\nu}}
\providecommand{\vxi}{\vec{\xi}}
\providecommand{\vpi}{\vec{\pi}}
\providecommand{\vrho}{\vec{\rho}}
\providecommand{\vsigma}{\vec{\sigma}}
\providecommand{\vtau}{\vec{\tau}}
\providecommand{\vphi}{\vec{\phi}}
\providecommand{\vvarphi}{\vec{\varphi}}
\providecommand{\vchi}{\vec{\chi}}
\providecommand{\vpsi}{\vec{\psi}}
\providecommand{\vomega}{\vec{\omega}}









% Tilde
\providecommand{\wtilde}{\widetilde{w}}




% Tilde Matrix / Vector
\providecommand{\mAtilde}{\mat{\widetilde{A}}}
\providecommand{\mDtilde}{\mat{\widetilde{D}}}
\providecommand{\mWtilde}{\mat{\widetilde{W}}}
\providecommand{\vftilde}{\boldsymbol{\widetilde{f}}}
\providecommand{\vvtilde}{\boldsymbol{\widetilde{v}}}
\providecommand{\vxtilde}{\boldsymbol{\widetilde{x}}}
\providecommand{\vztilde}{\boldsymbol{\widetilde{z}}}

% Hat
\providecommand{\fhat}{\widehat{f}}
\providecommand{\zhat}{\widehat{z}}
\providecommand{\chat}{\widehat{c}}
\providecommand{\sigmahat}{\widehat{\sigma}}
\providecommand{\thetahat}{\widehat{\theta}}
\providecommand{\lambdahat}{\widehat{\lambda}}

% Hat Matrix / Vector
\providecommand{\vfhat}{\boldsymbol{\widehat{f}}}
\providecommand{\vzhat}{\boldsymbol{\widehat{z}}}
\providecommand{\vchat}{\boldsymbol{\widehat{c}}}
\providecommand{\vhat}{\widehat{v}}
\providecommand{\mAhat}{\mat{\widehat{A}}}
\providecommand{\vxhat}{\boldsymbol{\widehat{x}}}
\providecommand{\vuhat}{\boldsymbol{\widehat{u}}}
\providecommand{\vvhat}{\boldsymbol{\widehat{v}}}
\providecommand{\vubar}{\boldsymbol{\bar{u}}}
\providecommand{\vthetahat}{\boldsymbol{\widehat{\theta}}}
\providecommand{\vlambdahat}{\boldsymbol{\widehat{\lambda}}}


% Star
\providecommand{\fstar}{f^*}






% Standard 0 and 1
\providecommand{\vzero}{\vec{0}}
\providecommand{\vone}{\vec{1}}






% Operators
\providecommand{\conv}{\ast}
\providecommand{\circonv}[1]{\circledast_{#1}}
\providecommand{\Var}{\mathrm{Var}}
\newcommand{\floor}[1]{\left \lfloor #1 \right \rfloor}
\newcommand{\ceil}[1]{\left \lceil #1 \right \rceil}
\newcommand{\round}[1]{\left \lceil #1 \right \rfloor}

% Texts
\newcommand{\defequal}{\mathop{\overset{\mbox{\tiny{def}}}{=}}}
\newcommand{\subjectto}{\mathop{\mathrm{subject\, to}}}
\newcommand{\argmin}[1]{\mathop{\underset{#1}{\mbox{argmin}}}}
\newcommand{\argmax}[1]{\mathop{\underset{#1}{\mbox{argmax}}}}
\newcommand{\minimize}[1]{\mathop{\underset{#1}{\mathrm{minimize}}}}
\newcommand{\maximize}[1]{\mathop{\underset{#1}{\mathrm{maximize}}}}
\newcommand{\diag}[1]{\mathop{\mathrm{diag}\left\{#1\right\}}}
\newcommand{\MSE}{\mathrm{MSE}}
\newcommand{\trace}[1]{\mathop{\mathrm{Tr}\left\{#1\right\}}}
\newcommand{\erf}{\mbox{erf}}
\providecommand{\SNRH}{\mbox{SNR}_{\text{H}}}



%\newgray{Gray08}{0.8}
%\newgray{Gray07}{0.7}
%\newgray{Gray06}{0.6}
%\newgray{Gray05}{0.5}

